Contrastive Self-Supervised Network Intrusion Detection using Augmented Negative Pairs

Network intrusion detection remains a critical challenge in cybersecurity. While supervised machine learning models achieve state-of-the-art performance, their reliance on large labelled datasets makes them impractical for many real-world applications. Anomaly detection methods, which train exclusively on benign traffic to identify malicious activity, suffer from high false positive rates, limiting their usability. Recently, self-supervised learning techniques have demonstrated improved performance with lower false positive rates by learning discriminative latent representations of benign traffic. In particular, contrastive self-supervised models achieve this by minimizing the distance between similar (positive) views of benign traffic while maximizing it between dissimilar (negative) views. Existing approaches generate positive views through data augmentation and treat other samples as negative. In contrast, this work introduces Contrastive Learning using Augmented Negative pairs (CLAN), a novel paradigm for network intrusion detection where augmented samples are treated as negative views - representing potentially malicious distributions - while other benign samples serve as positive views. This approach enhances both classification accuracy and inference efficiency after pretraining on benign traffic. Experimental evaluation on the Lycos2017 dataset demonstrates that the proposed method surpasses existing self-supervised and anomaly detection techniques in a binary classification task. Furthermore, when fine-tuned on a limited labelled dataset, the proposed approach achieves superior multi-class classification performance compared to existing self-supervised models.

==> diagrams/embedding_comp/clanp_embeddings_tikz.tex <==
\begin{tikzpicture}
    % Define styles
    \tikzset{
        point/.style = {circle, draw=black, fill=#1, inner sep=0pt, minimum width=4pt},
        label/.style = {text width=2cm, align=center},
        cross/.style n args={1}{
            cross out, draw=black,
            inner sep=0pt, outer sep=0pt,
            minimum size={2*(#1-\pgflinewidth)}
        },
        measure/.style = {draw, <->, thick}
    }
    
    % centroid
    \node[cross=4,black, anchor = center] at (0,0) {};

    % draw boundaries
    \draw[dashed, black, thick] (0,0) circle [radius=0.95];
    \draw[dashed, black, thick] (0,0) circle [radius=1.88];
    \draw[dashed, black, thick] (0,0) circle [radius=2.81];

    % Blue cluster points
    \node[point=blue] (b1) at (0.99, -0.40) {};
    \node[point=blue] (b2) at (-1.30, 0.49) {};
    \node[point=blue] (b6) at (0.68, -0.88) {};
    \node[point=blue] (b7) at (-0.36, -0.75) {};
    \node[point=blue] (b8) at (-1.00, 0.76) {};
    \node[point=blue] (b9) at (0.34, 1.23) {};
    \node[point=blue] (b11) at (-0.66, 0.39) {};
    \node[point=blue] (b12) at (0.93, -0.78) {};
    \node[point=blue] (b13) at (-1.19, -0.15) {};
    \node[point=blue] (b17) at (-0.35, 1.24) {};
    \node[point=blue] (b19) at (0.06, -1.29) {};
    \node[point=blue] (b20) at (-1, -0.8) {};
    \node[point=blue] (b21) at (0.5,0.25) {};
    \node[point=blue] at (0.74, 0.11) {};
    \node[point=blue] at (-1.12, -0.01) {};
    \node[point=blue] at (0.84, -0.05) {};
    \node[point=blue] at (-0.62, -0.28) {};
    \node[point=blue] at (1.38, -0.48) {};
    \node[point=blue] at (-0.74, 1.06) {};
    \node[point=blue] at (2.20, -0.11) {};
    \node[point=blue] at (0.95, 0.31) {};
    \node[point=blue] at (0.99, 0.17) {};
    \node[point=blue] at (1.48, -0.66) {};
    \node[point=blue] at (-0.44, -0.78) {};
    \node[point=blue] at (1.23, -0.81) {};
    \node[point=blue] at (0.69, -0.46) {};
    \node[point=blue] at (-1.36, -1.02) {};
    \node[point=blue] at (1.24, -1.06) {};
    \node[point=blue] at (-0.67, 1.76) {};
    \node[point=blue] at (0.48, -0.81) {};
    \node[point=blue] at (0.95, 0.16) {};
    \node[point=blue] at (0.79, 0.72) {};
    
    % Red cluster points
    \node[point=red] (r0) at (-2.10, -2.42) {};
    \node[point=red] (r1) at (0.41, 3.03) {};
    \node[point=red] (r2) at (-1.12, 3.59) {};
    \node[point=red] (r3) at (3.13, 0.79) {};
    \node[point=red] (r4) at (0.41, -3.07) {};
    \node[point=red] (r5) at (-3.65, 1.62) {};
    \node[point=red] (r6) at (-2.52, -1.97) {};
    \node[point=red] (r7) at (-3.14, 0.68) {};
    \node[point=red] (r8) at (3.11, 1.94) {};
    \node[point=red] (r9) at (2.81, 1.17) {};
    \node[point=red] (r10) at (-2.49, 2.37) {};
    \node[point=red] (r11) at (3.38, -0.18) {};
    \node[point=red] (r12) at (2.81, -1.61) {};
    \node[point=red] (r13) at (-3.13, 1.39) {};
    \node[point=red] (r14) at (3.54, 1.57) {};
    \node[point=red] (r15) at (-0.64, 3.21) {};
    \node[point=red] (r16) at (0.24, -3.07) {};
    \node[point=red] (r17) at (-2.88, 1.57) {};
    \node[point=red] (r18) at (-3.43, 0.29) {};
    \node[point=red] (r19) at (-0.94, -3.17) {};
    \node[point=red] (r20) at (-2.10, -2.35) {};
    \node[point=red] (r21) at (2.97, 0.45) {};
    \node[point=red] (r22) at (-2.95, -2.03) {};
    \node[point=red] (r23) at (-2.29, -2.08) {};
    \node[point=red] (r24) at (0.84, 3.28) {};
    \node[point=red] (r25) at (2.39, -1.93) {};
    \node[point=red] (r26) at (1.26, -2.93) {};
    \node[point=red] (r27) at (3.01, -0.29) {};
    \node[point=red] (r28) at (-0.86, -3.11) {};
    \node[point=red] (r29) at (3.18, -0.16) {};
    \node[point=red] (r30) at (2.81, 1.10) {};
    \node[point=red] (r31) at (-3.18, 0.80) {};
    \node[point=red] (r32) at (2.35, -2.03) {};
    \node[point=red] (r33) at (3.44, 0.69) {};
    \node[point=red] (r34) at (-2.59, 1.68) {};
    \node[point=red] (r35) at (-0.60, 3.27) {};
    \node[point=red] (r36) at (-3.20, -0.37) {};
    \node[point=red] (r37) at (3.37, 0.38) {};
    \node[point=red] (r38) at (3.72, -1.26) {};
    \node[point=red] (r39) at (1.08, -2.80) {};
    \node[point=red] (r40) at (-3.97, -1.38) {};
    \node[point=red] (r41) at (-0.85, -3.19) {};
    \node[point=red] (r42) at (-3.05, 0.89) {};
    \node[point=red] (r43) at (0.44, 4.01) {};
    \node[point=red] (r44) at (2.95, 0.74) {};
    \node[point=red] (r45) at (0.52, 2.96) {};
    \node[point=red] (r46) at (-1.65, -3.21) {};
    \node[point=red] (r47) at (2.98, -0.79) {};
    \node[point=red] (r48) at (3.21, 0.82) {};
    \node[point=red] (r49) at (0.90, 2.96) {};
    \node[point=red] (r50) at (-1.19, -2.95) {};
    \node[point=red] (r51) at (3.02, 1.66) {};
    \node[point=red] (r52) at (2.88, -1.17) {};
    \node[point=red] (r53) at (-3.73, 0.56) {};
    \node[point=red] (r54) at (3.03, 0.47) {};
    \node[point=red] (r55) at (-1.74, 2.50) {};
    \node[point=red] (r56) at (3.73, -0.21) {};
    \node[point=red] (r57) at (3.24, -1.01) {};
    \node[point=red] (r58) at (-2.62, -1.79) {};
    \node[point=red] (r59) at (-2.78, 1.58) {};
    \node[point=red] (r60) at (0.37, 3.02) {};
    \node[point=red] (r61) at (-2.02, 2.90) {};
    \node[point=red] (r62) at (-1.18, 2.97) {};
    \node[point=red] (r63) at (3.70, -0.34) {};
    \node[point=red] (r64) at (-1.18, 2.81) {};
    \node[point=red] (r65) at (2.30, -2.08) {};
    \node[point=red] (r66) at (-0.22, 3.04) {};
    \node[point=red] (r67) at (-1.40, 3.23) {};
    \node[point=red] (r68) at (3.46, -0.17) {};
    \node[point=red] (r69) at (-0.08, -3.09) {};
    \node[point=red] (r70) at (3.45, -0.73) {};
    \node[point=red] (r71) at (-1.76, 2.47) {};
    \node[point=red] (r72) at (1.84, -2.45) {};
    \node[point=red] (r73) at (1.55, 2.74) {};
    \node[point=red] (r74) at (0.99, 3.01) {};
    \node[point=red] (r75) at (-3.17, 1.62) {};
    \node[point=red] (r76) at (-3.20, 0.27) {};
    \node[point=red] (r77) at (-2.31, -2.27) {};
    \node[point=red] (r78) at (1.25, 3.14) {};
    \node[point=red] (r79) at (-2.47, -1.84) {};
    \node[point=red] (r80) at (-0.14, -3.53) {};
    \node[point=red] (r81) at (2.45, 1.84) {};
    \node[point=red] (r82) at (1.98, -2.43) {};
    \node[point=red] (r83) at (2.98, 1.33) {};
    \node[point=red] (r84) at (-2.87, 1.63) {};
    
\end{tikzpicture}

==> diagrams/embedding_comp/ssl_embedding_tikz.tex <==
\begin{tikzpicture}
    \useasboundingbox (-2.5, -2.5) rectangle (2.7, 2);
    % Define styles
    \tikzset{
        point/.style = {circle, draw=black, fill=#1, inner sep=0pt, minimum width=4pt},
        label/.style = {text width=2cm, align=center},
        cross/.style n args={1}{
            cross out, draw=black,
            inner sep=0pt, outer sep=0pt,
            minimum size={2*(#1-\pgflinewidth)}
        },
        measure/.style = {draw, <->, thick}
    }
    

    % -- centeroids 
    \node[point=blue, anchor = center] (b0) at (0.0, 1.0) {};
    \node[point=blue, anchor = center] (b1) at (-1.2, -0.2) {};
    \node[point=blue, anchor = center] (b2) at (1.0, 0.0) {};
    \node[point=blue, anchor = center] (b3) at (0.8, -1.2) {};

    % -- contours
    \foreach \x/\y in {0.0/1.0, -1.2/-0.2, 1.0/0.0, 0.8/-1.2} {
        \draw[dashed, black, thick] (\x,\y) circle [radius=0.27];
        \draw[dashed, black, thick] (\x,\y) circle [radius=.535];
        \draw[dashed, black, thick] (\x,\y) circle [radius=0.8];
    }


    % -- Orange Points
    \node[point=orange] (o0) at (-0.19, 0.68) {};
    \node[point=orange] (o1) at (-0.15, 0.82) {};
    \node[point=orange] (o2) at (0.5, 1.21) {};
    \node[point=orange] (o10) at (-0.48, 1.19) {};
    \node[point=orange] (o12) at (0.33, 1.18) {};
    \node[point=orange] (o13) at (0.01, 1.63) {};
    \node[point=orange] (o14) at (0.18, 0.9) {};
    \node[point=orange] (o15) at (-0.31, 0.81) {};
    \node[point=orange] (o16) at (-1.15, -0.57) {};
    \node[point=orange] (o17) at (-0.92, -0.09) {};
    \node[point=orange] (o18) at (-1.1, 0.16) {};
    \node[point=orange] (o19) at (-1.47, -0.28) {};
    \node[point=orange] (o20) at (-1.74, -0.09) {};
    \node[point=orange] (o21) at (-1.45, 0.07) {};
    \node[point=orange] (o22) at (-1.6, -0.1) {};
    \node[point=orange] (o23) at (-1.14, 0.25) {};
    \node[point=orange] (o24) at (-1.39, 0.44) {};
    \node[point=orange] (o25) at (-1.38, -0.09) {};
    \node[point=orange] (o26) at (-0.94, -0.15) {};
    \node[point=orange] (o27) at (-1.3, -0.02) {};
    \node[point=orange] (o28) at (-1.16, 0.16) {};
    \node[point=orange] (o29) at (-1.89, 0.08) {};
    \node[point=orange] (o30) at (-0.94, -0.06) {};
    \node[point=orange] (o31) at (-0.98, -0.29) {};
    \node[point=orange] (o32) at (-1.22, 0.25) {};
    \node[point=orange] (o33) at (1.21, -0.31) {};
    \node[point=orange] (o34) at (1.08, -0.54) {};
    \node[point=orange] (o35) at (1.18, 0.45) {};
    \node[point=orange] (o36) at (0.73, 0.12) {};
    \node[point=orange] (o37) at (0.84, -0.41) {};
    \node[point=orange] (o38) at (1.29, -0.25) {};
    \node[point=orange] (o39) at (1.06, 0.23) {};
    \node[point=orange] (o40) at (0.6, -0.23) {};
    \node[point=orange] (o41) at (1.2, -0.19) {};
    \node[point=orange] (o42) at (0.76, 0.44) {};
    \node[point=orange] (o43) at (1.18, 0.17) {};
    \node[point=orange] (o44) at (0.63, 0.23) {};
    \node[point=orange] (o45) at (0.97, 0.4) {};
    \node[point=orange] (o46) at (1.39, -0.19) {};
    \node[point=orange] (o47) at (1.15, 0.15) {};
    \node[point=orange] (o48) at (0.87, -0.27) {};
    \node[point=orange] (o49) at (1.47, 0.0) {};
    \node[point=orange] (o50) at (1.28, -0.09) {};
    \node[point=orange] (o51) at (1.11, -1.73) {};
    \node[point=orange] (o52) at (0.39, -0.96) {};
    \node[point=orange] (o53) at (0.58, -1.13) {};
    \node[point=orange] (o54) at (0.24, -1.62) {};
    \node[point=orange] (o55) at (0.46, -1.09) {};
    \node[point=orange] (o56) at (0.92, -1.47) {};
    \node[point=orange] (o58) at (1.32, -1.7) {};
    \node[point=orange] (o59) at (1.21, -1.3) {};
    \node[point=orange] (o60) at (0.99, -1.46) {};
    \node[point=orange] (o61) at (0.73, -0.77) {};
    \node[point=orange] (o62) at (0.86, -0.5) {};
    \node[point=orange] (o63) at (1.2, -1.17) {};
    \node[point=orange] (o64) at (1.29, -1.35) {};
    
    % Red points (outliers outside the contours)
    \node[point=red] at (-1.78, 0.75) {};
    \node[point=red] at (-0.12, -0.83) {};
    \node[point=red] at (-1.56, 1.10) {};
    \node[point=red] at (-0.8, 1.8) {};
    \node[point=red] at (-1.00, 1.66) {};
    \node[point=red] at (-2.10, -1.61) {};
    \node[point=red] at (-2.77, -0.59) {};
    \node[point=red] at (-0.63, -1.78) {};
    \node[point=red] at (1.68, 1.54) {};
    \node[point=red] at (2.83, -0.38) {};
    \node[point=red] at (2.36, 1.09) {};
    \node[point=red] at (-0.78, 0.37) {};
    \node[point=red] at (1.90, 1.09) {};
    \node[point=red] at (1.37, -2) {};
    \node[point=red] at (0.18, -2.2) {};
    \node[point=red] at (2.45, -0.83) {};
    \node[point=red] at (1.59, -2.4) {};
    \node[point=red] at (2.19, -0.08) {};

\end{tikzpicture}

==> diagrams/system_overview/centroid.tex <==
\begin{tikzpicture}
    % Define styles
    \tikzset{
        point/.style = {circle, draw=black, fill=#1, inner sep=0pt, minimum width=4pt},
        label/.style = {text width=2cm, align=center},
        cross/.style n args={1}{
            cross out, draw=black,
            inner sep=0pt, outer sep=0pt,
            minimum size={2*(#1-\pgflinewidth)}
        },
        measure/.style = {draw, <->, thick}
    }
    
    % Draw the cross at the center
    \node[cross=4,black, anchor = center] at (0,0) {};
    
    % Draw concentric circles
    \draw[dashed, black, thick, anchor = center] (0,0) circle [radius=3];
    \draw[dashed, black, thick, anchor = center] (0,0) circle [radius=1.5];
\end{tikzpicture}


==> diagrams/system_overview/clad_embeddings.tex <==
\begin{tikzpicture}
    % Define styles
    \tikzset{
        point/.style = {circle, draw=black, fill=#1, inner sep=0pt, minimum width=4pt},
        label/.style = {text width=2cm, align=center},
        cross/.style n args={1}{
            cross out, draw=black,
            inner sep=0pt, outer sep=0pt,
            minimum size={2*(#1-\pgflinewidth)}
        },
        measure/.style = {draw, <->, thick}
    }
    
    % Blue cluster points
    \node[point=blue] (b1) at (0.99, -0.40) {};
    \node[point=blue] (b2) at (-1.30, 0.49) {};
    %\node[point=blue] (b5) at (-0.67, 0.54) {};
    \node[point=blue] (b6) at (0.68, -0.88) {};
    \node[point=blue] (b7) at (-0.36, -0.75) {};
    \node[point=blue] (b8) at (-1.00, 0.76) {};
    \node[point=blue] (b9) at (0.34, 1.23) {};
    \node[point=blue] (b11) at (-0.66, 0.39) {};
    \node[point=blue] (b12) at (0.93, -0.78) {};
    \node[point=blue] (b13) at (-1.19, -0.15) {};
    \node[point=blue] (b17) at (-0.35, 1.24) {};
    \node[point=blue] (b19) at (0.06, -1.29) {};
    \node[point=blue] (b20) at (-1, -0.8) {};
    \node[point=blue] (b21) at (0.5,0.25) {};
    
    
    % Red cluster points
    \node[point=red] (r0) at (-2.10, -2.42) {};
    \node[point=red] (r1) at (0.41, 3.03) {};
    \node[point=red] (r2) at (-1.12, 3.59) {};
    \node[point=red] (r3) at (3.13, 0.79) {};
    \node[point=red] (r4) at (0.41, -3.07) {};
    \node[point=red] (r5) at (-3.65, 1.62) {};
    \node[point=red] (r6) at (-2.52, -1.97) {};
    \node[point=red] (r7) at (-3.14, 0.68) {};
    \node[point=red] (r8) at (3.11, 1.94) {};
    \node[point=red] (r9) at (2.81, 1.17) {};
    \node[point=red] (r10) at (-2.49, 2.37) {};
    \node[point=red] (r11) at (3.38, -0.18) {};
    \node[point=red] (r12) at (2.81, -1.61) {};
    \node[point=red] (r13) at (-3.13, 1.39) {};
    \node[point=red] (r14) at (3.54, 1.57) {};
    \node[point=red] (r15) at (-0.64, 3.21) {};
    \node[point=red] (r16) at (0.24, -3.07) {};
    \node[point=red] (r17) at (-2.88, 1.57) {};
    \node[point=red] (r18) at (-3.43, 0.29) {};
    \node[point=red] (r19) at (-0.94, -3.17) {};
    \node[point=red] (r20) at (-2.10, -2.35) {};
    \node[point=red] (r21) at (2.97, 0.45) {};
    \node[point=red] (r22) at (-2.95, -2.03) {};
    \node[point=red] (r23) at (-2.29, -2.08) {};
    \node[point=red] (r24) at (0.84, 3.28) {};
    \node[point=red] (r25) at (2.39, -1.93) {};
    \node[point=red] (r26) at (1.26, -2.93) {};
    \node[point=red] (r27) at (3.01, -0.29) {};
    \node[point=red] (r28) at (-0.86, -3.11) {};
    \node[point=red] (r29) at (3.18, -0.16) {};
    \node[point=red] (r30) at (2.81, 1.10) {};
    \node[point=red] (r31) at (-3.18, 0.80) {};
    \node[point=red] (r32) at (2.35, -2.03) {};
    \node[point=red] (r33) at (3.44, 0.69) {};
    \node[point=red] (r34) at (-2.59, 1.68) {};
    \node[point=red] (r35) at (-0.60, 3.27) {};
    \node[point=red] (r36) at (-3.20, -0.37) {};
    \node[point=red] (r37) at (3.37, 0.38) {};
    \node[point=red] (r38) at (3.72, -1.26) {};
    \node[point=red] (r39) at (1.08, -2.80) {};
    \node[point=red] (r40) at (-3.97, -1.38) {};
    \node[point=red] (r41) at (-0.85, -3.19) {};
    \node[point=red] (r42) at (-3.05, 0.89) {};
    \node[point=red] (r43) at (0.44, 4.01) {};
    \node[point=red] (r44) at (2.95, 0.74) {};
    \node[point=red] (r45) at (0.52, 2.96) {};
    \node[point=red] (r46) at (-1.65, -3.21) {};
    \node[point=red] (r47) at (2.98, -0.79) {};
    \node[point=red] (r48) at (3.21, 0.82) {};
    \node[point=red] (r49) at (0.90, 2.96) {};
    \node[point=red] (r50) at (-1.19, -2.95) {};
    \node[point=red] (r51) at (3.02, 1.66) {};
    \node[point=red] (r52) at (2.88, -1.17) {};
    \node[point=red] (r53) at (-3.73, 0.56) {};
    \node[point=red] (r54) at (3.03, 0.47) {};
    \node[point=red] (r55) at (-1.74, 2.50) {};
    \node[point=red] (r56) at (3.73, -0.21) {};
    \node[point=red] (r57) at (3.24, -1.01) {};
    \node[point=red] (r58) at (-2.62, -1.79) {};
    \node[point=red] (r59) at (-2.78, 1.58) {};
    \node[point=red] (r60) at (0.37, 3.02) {};
    \node[point=red] (r61) at (-2.02, 2.90) {};
    \node[point=red] (r62) at (-1.18, 2.97) {};
    \node[point=red] (r63) at (3.70, -0.34) {};
    \node[point=red] (r64) at (-1.18, 2.81) {};
    \node[point=red] (r65) at (2.30, -2.08) {};
    \node[point=red] (r66) at (-0.22, 3.04) {};
    \node[point=red] (r67) at (-1.40, 3.23) {};
    \node[point=red] (r68) at (3.46, -0.17) {};
    \node[point=red] (r69) at (-0.08, -3.09) {};
    \node[point=red] (r70) at (3.45, -0.73) {};
    \node[point=red] (r71) at (-1.76, 2.47) {};
    \node[point=red] (r72) at (1.84, -2.45) {};
    \node[point=red] (r73) at (1.55, 2.74) {};
    \node[point=red] (r74) at (0.99, 3.01) {};
    \node[point=red] (r75) at (-3.17, 1.62) {};
    \node[point=red] (r76) at (-3.20, 0.27) {};
    \node[point=red] (r77) at (-2.31, -2.27) {};
    \node[point=red] (r78) at (1.25, 3.14) {};
    \node[point=red] (r79) at (-2.47, -1.84) {};
    \node[point=red] (r80) at (-0.14, -3.53) {};
    \node[point=red] (r81) at (2.45, 1.84) {};
    \node[point=red] (r82) at (1.98, -2.43) {};
    \node[point=red] (r83) at (2.98, 1.33) {};
    \node[point=red] (r84) at (-2.87, 1.63) {};
    %\node[point=red] (r85) at (2.31, -3.00) {};
    \node[point=red] (r86) at (2.33, 1.96) {};
    \node[point=red] (r87) at (-2.53, 2.08) {};
    \node[point=red] (r88) at (-3.03, -0.62) {};
    \node[point=red] (r89) at (0.06, -3.03) {};
    \node[point=red] (r90) at (-0.77, 3.00) {};
    \node[point=red] (r91) at (-0.32, -2.99) {};
    \node[point=red] (r92) at (-2.63, 1.72) {};
    \node[point=red] (r93) at (0.51, 3.05) {};
    \node[point=red] (r94) at (2.12, 2.77) {};
    \node[point=red] (r95) at (-3.32, 0.85) {};
    \node[point=red] (r96) at (0.02, 3.41) {};
    \node[point=red] (r97) at (-3.52, -0.97) {};
    \node[point=red] (r98) at (2.37, -1.96) {};
    \node[point=red] (r99) at (-2.89, -1.49) {};

    % draw boundaries
    \draw[dashed, black, thick] (0,0) circle [radius=3];
    \draw[dashed, black, thick] (0,0) circle [radius=1.5];
\end{tikzpicture}
